Minimax Mixing Time of the Metropolis-Adjusted Langevin Algorithm for Log-Concave Sampling

We study the mixing time of the Metropolis-adjusted Langevin algorithm (MALA) for sampling from a log-smooth and strongly log-concave distribution. We establish its optimal minimax mixing time under a warm start. Our main contribution is two-fold. First, for a $d$-dimensional log-concave density with condition number $\kappa$, we show that MALA with a warm start mixes in $\tilde O(\kappa \sqrt{d})$ iterations up to logarithmic factors. This improves upon the previous work on the dependency of either the condition number $\kappa$ or the dimension $d$. Our proof relies on comparing the leapfrog integrator with the continuous Hamiltonian dynamics, where we establish a new concentration bound for the acceptance rate. Second, we prove a spectral gap based mixing time lower bound for reversible MCMC algorithms on general state spaces. We apply this lower bound result to construct a hard distribution for which MALA requires at least $\tilde \Omega (\kappa \sqrt{d})$ steps to mix. The lower bound for MALA matches our upper bound in terms of condition number and dimension. Finally, numerical experiments are included to validate our theoretical results.

==> macros.tex <==
%!TEX root = main.tex

\newcommand{\minimaxmixingtime}{\mathfrak{T}}
\newcommand{\dist}{\mathfrak{D}}
\newcommand{\constO}{\ensuremath{\varrho}}
\newcommand{\constC}{\ensuremath{C_\constO}}
\newcommand{\constc}{\ensuremath{c}}
\newcommand{\constUniversal}{\ensuremath{c_0}}
\newcommand{\constUniversall}{\ensuremath{c_1}}
\newcommand{\constUniversalll}{\ensuremath{c_2}}
\newcommand{\constUniversallll}{\ensuremath{c_3}}
\newcommand{\constUniversalllll}{\ensuremath{c_4}}
\newcommand{\integer}{\ensuremath{N}}
\newcommand{\constp}{\ensuremath{c_1}}

\newcommand{\constK}{\ensuremath{K_0}}
\newcommand{\constKK}{\ensuremath{K_1}}
\newcommand{\constKKK}{\ensuremath{K_2}}
\newcommand{\rc}{\ensuremath{{\color{red}c}}}
\newcommand{\todo}{\ensuremath{{\color{red}{???}}}}
\newcommand{\tmp}{\ensuremath{\Psi}}

\newcommand{\constg}{\ensuremath{\gamma}}

\newcommand{\bigO}{\ensuremath{O}}
\newcommand{\TTheta}{\tilde\Theta}
\newcommand{\TO}{\tilde O}
\newcommand{\TOmega}{\tilde \Omega}
\newcommand{\Remain}{\ensuremath{R}}

\newcommand{\statespace}{\ensuremath{\mathcal{X}}}
\newcommand{\initial}{\ensuremath{\mu_0}}
\newcommand{\diffusion}{\ensuremath{v}}

\newcommand{\coord}[2]{\ensuremath{#1_{[#2]}} }

% symbols about the algo and the density
\newcommand{\proposal}{\ensuremath{\mathcal{Q}}}
\newcommand{\transition}{\ensuremath{\mathcal{T}}}
\newcommand{\transitionS}{\ensuremath{K}}
\newcommand{\transitionbf}{\ensuremath{\mathcal{T}^{\text{before-lazy}}}}
\newcommand{\Kernel}{\mathcal{K}}
\newcommand{\kernel}{\ensuremath{K}}
\newcommand{\propkernel}{\ensuremath{Q}}
\newcommand{\targetdistri}{\ensuremath{\pi}}
\newcommand{\target}{\ensuremath{\pi}}
\newcommand{\targetf}{\ensuremath{f}}
\newcommand{\gradf}{\ensuremath{\nabla \targetf}}
\newcommand{\hessf}{\ensuremath{H}}
\newcommand{\dirichlet}{\ensuremath{\mathcal{E}}}
\newcommand{\accept}{\ensuremath{\mathcal{A}}}

\newcommand{\conductance}{\ensuremath{\Phi}}
\newcommand{\condS}{\ensuremath{\mathtt{s}}}

\newcommand{\isop}{\ensuremath{\psi}}
\newcommand{\lazy}{\ensuremath{\omega}}


% hat version
\newcommand{\hq}{\ensuremath{\hat q}}
% continuous version
\newcommand{\cq}{\ensuremath{q}}
\newcommand{\hp}{\ensuremath{\hat p}}
\newcommand{\cp}{\ensuremath{p}}
% interpolate version
\newcommand{\tq}{\ensuremath{\tilde{q}}}

\newcommand{\normp}{\ensuremath{\vecnorm{\cp_0}{2}}}
\newcommand{\normgradq}{\ensuremath{\vecnorm{\gradf(\cq_0)}{2}}}

% key term in the accept reject
\newcommand{\arkey}{\ensuremath{B}}
\newcommand{\arkpower}{\ensuremath{D}}
\newcommand{\keycross}{\ensuremath{J}}
% shorthand for gradf(y - \alpha^2/2 gradf(y))
\newcommand{\gradshift}{\ensuremath{g}}

% proof related
\newcommand{\interG}{\ensuremath{G}}
\newcommand{\interR}{\ensuremath{R}}
% \newcommand{\goodqset}{\ensuremath{\Omega}}
% \newcommand{\goodpset}{\ensuremath{\Lambda}}
% \newcommand{\goodpqset}{\ensuremath{\Lambda}}
\newcommand{\goodqpset}{\ensuremath{\Lambda}}
\newcommand{\goodqsetcond}{\ensuremath{\Upsilon}}

\newcommand{\Exsqp}{\ensuremath{\Exs_{\cq_0 \sim \target, \cp_0 \sim \Normal(0, \Ind_\dims)}}}
\newcommand{\Exsq}{\ensuremath{\Exs_{\cq_0 \sim \target}}}
\newcommand{\Exsp}{\ensuremath{\Exs_{\cp_0 \sim \Normal(0, \Ind_\dims)}}}



% parameters
\newcommand{\smoothparam}{\ensuremath{L}}
\newcommand{\scparam}{\ensuremath{m}}
\newcommand{\condi}{\ensuremath{\kappa}}
\newcommand{\warmparam}{\ensuremath{M}}
\newcommand{\step}{\ensuremath{\eta}}
\newcommand{\tole}{\ensuremath{\epsilon}}
\newcommand{\deltaf}{\ensuremath{\delta}}
\newcommand{\deltas}{\ensuremath{\theta}}
\newcommand{\Deltapart}{\ensuremath{\Delta}}
\newcommand{\loExpo}{\ensuremath{\zeta}}

\newcommand{\hula}{h_{\mathrm{ULA}}}
\newcommand{\nula}{{N_{\mathrm{ULA}}}}
\newcommand{\hulaf}{{h_1}}%{h_{\mathrm{ULA},1}}
\newcommand{\nulaf}{{N_1}}%{{N_{\mathrm{ULA},1}}}
\newcommand{\hulas}{{h_2}}%{h_{\mathrm{ULA},2}}
\newcommand{\nulas}{{N_2}}%{{N_{\mathrm{ULA},2}}}
\newcommand{\hmala}{{h_3}}%{h_{\mathrm{MALA}}}
\newcommand{\nmala}{{N_3}}%{{N_{\mathrm{MALA}}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% set margins
\setlength{\textwidth}{\paperwidth}
\addtolength{\textwidth}{-6cm}
\setlength{\textheight}{\paperheight}
\addtolength{\textheight}{-4cm}
\addtolength{\textheight}{-1.1\headheight}
\addtolength{\textheight}{-\headsep}
\addtolength{\textheight}{-\footskip}
\setlength{\oddsidemargin}{0.5cm}
\setlength{\evensidemargin}{0.5cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Basic Terms like defn, etal, polylog %%%%%%%%%%%
\newcommand{\defn}{:=}
\newcommand{\rdefn}{=:}
\newcommand{\etal}{{et al.}}
\newcommand{\polylog}{\text{poly-log}}
\newcommand{\polylogfactor}{\kappa_{\obs, \dims}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%% Theorem related %%%%%%%%%%%

% \newtheoremstyle{named}{}{}{\itshape}{}{\bfseries}{.}{.5em}{\thmnote{#3's }#1}
% \theoremstyle{named}
% \newtheorem*{namedtheorem}{Lemma}

% %%%%%%%
% \theoremstyle{plain}

% % {Theorem, Proposition, Lemma, Corollary} numbered sequentially
% % throughout the paper
% \newtheorem{theorem}{Theorem}
% \newtheorem{proposition}{Proposition}
% \newtheorem{lemma}{Lemma}
% \newtheorem{corollary}{Corollary}
% \newtheorem{definition}{Definition}
% \newtheorem{conjecture}{Conjecture}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% WIDEBAR COMMAND
\newlength{\widebarargwidth}
\newlength{\widebarargheight}
\newlength{\widebarargdepth}
\DeclareRobustCommand{\widebar}[1]{%
  \settowidth{\widebarargwidth}{\ensuremath{#1}}%
  \settoheight{\widebarargheight}{\ensuremath{#1}}%
  \settodepth{\widebarargdepth}{\ensuremath{#1}}%
  \addtolength{\widebarargwidth}{-0.3\widebarargheight}%
  \addtolength{\widebarargwidth}{-0.3\widebarargdepth}%
  \makebox[0pt][l]{\hspace{0.3\widebarargheight}%
    \hspace{0.3\widebarargdepth}%
    \addtolength{\widebarargheight}{0.3ex}%
    \rule[\widebarargheight]{0.95\widebarargwidth}{0.1ex}}%
  {#1}}



%%% New version of \caption puts things in smaller type, single-spaced
%%% and indents them to set them off more from the text.
\makeatletter
\long\def\@makecaption#1#2{
        \vskip 0.8ex
        \setbox\@tempboxa\hbox{\small {\bf #1:} #2}
        \parindent 1.5em  %% How can we use the global value of this???
        \dimen0=\hsize
        \advance\dimen0 by -3em
        \ifdim \wd\@tempboxa >\dimen0
                \hbox to \hsize{
                        \parindent 0em
                        \hfil
                        \parbox{\dimen0}{\def\baselinestretch{0.96}\small
                                {\bf #1.} #2
                                %%\unhbox\@tempboxa
                                }
                        \hfil}
        \else \hbox to \hsize{\hfil \box\@tempboxa \hfil}
        \fi
        }
\makeatother



%% COMMENTING commands

\long\def\comment#1{}
\definecolor{battleshipgrey}{rgb}{0.52, 0.52, 0.51}
\definecolor{darkgray}{rgb}{0.66, 0.66, 0.66}
\definecolor{darkgreen}{rgb}{0.0, 0.2, 0.13}
\definecolor{darkspringgreen}{rgb}{0.09, 0.45, 0.27}
\definecolor{dukeblue}{rgb}{0.0, 0.0, 0.61}
\definecolor{olivedrab7}{rgb}{0.24, 0.2, 0.12}
\definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
\definecolor{darkscarlet}{rgb}{0.34, 0.01, 0.1}
\definecolor{candyapplered}{rgb}{1.0, 0.03, 0.0}
\definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
\definecolor{applegreen}{rgb}{0.55, 0.71, 0.0}

\newcommand{\red}[1]{\textcolor{red}{#1}}
\newcommand{\mjwcomment}[1]{{\bf{{\red{{MJW --- #1}}}}}}
\newcommand{\blue}[1]{\textcolor{blue}{#1}}
\newcommand{\green}[1]{\textcolor{green}{#1}}
\newcommand{\highlight}[1]{\textcolor{applegreen}{#1}}
\newcommand{\yccomment}[1]{{\bf{{\red{{YC --- #1}}}}}}
\newcommand{\kwcomment}[1]{{\bf{{\blue{{KW --- #1}}}}}}
\newcommand{\kw}[1]{{\bf{{\blue{{#1}}}}}}


% \DeclareMathOperator{\det}{det}
\DeclareMathOperator{\modd}{mod}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\var}{var}
\DeclareMathOperator{\cov}{cov}
\DeclareMathOperator{\trace}{trace}
\DeclareMathOperator{\abs}{abs}
\DeclareMathOperator{\floor}{floor}
\DeclareMathOperator{\vol}{vol}
\DeclareMathOperator{\child}{child}
\DeclareMathOperator{\parent}{parent}
\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\toeplitz}{toeplitz}


% Basic Math notations
% Dimension etc.
\newcommand{\dims}{\ensuremath{d}}
\newcommand{\real}{\ensuremath{\mathbb{R}}}
\newcommand{\reald}{\ensuremath{{\real^\dims}}}
\newcommand{\naturalnum}{\ensuremath{\mathbb{N}}}
\newcommand{\Ind}{\ensuremath{\mathbb{I}}}
% Probability
\newcommand{\borel}{\ensuremath{\mathcal{B}}}
\newcommand{\lebesgue}{\ensuremath{\mathfrak{L}}}
\newcommand{\powerset}{\ensuremath{\mathfrak{P}}}
\newcommand{\lebesguemeasure}{\ensuremath{\lambda}}
\newcommand{\ball}{\ensuremath{\mathbb{B}}}
\newcommand{\Exs}{\ensuremath{{\mathbb{E}}}}
\newcommand{\Prob}{\ensuremath{{\mathbb{P}}}}
\newcommand{\Law}{\mathcal{L}}
\newcommand{\Normal}{\ensuremath{\mathcal{N}}}
\newcommand{\Ber}{\ensuremath{\mbox{Ber}}}
\newcommand{\Ent}{\text{Ent}}
\newcommand{\Var}{\ensuremath{{\rm Var}}}

\newcommand{\densityNormal}{\ensuremath{\varphi}}

% distribution distances
% KL divergence
\DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\kldiv}{\text{KL}\infdivx}
% tv distance
% \newcommand{\tvnorm}[1]{\ensuremath{ #1\|_{\mbox{\tiny{TV}}}}}
\newcommand{\tvdist}[2]{\ensuremath{ \mathtt{d}_{\textup{\tiny{TV}}}\parenth{#1, #2} }}
\newcommand{\chidist}[2]{\ensuremath{ \mathtt{d}_{2}\parenth{#1, #2} }}
\newcommand{\pdist}[3]{\ensuremath{ \mathtt{d}_{#1}\parenth{#2, #3} }}

\newcommand{\tvmix}[2]{\ensuremath{\mathtt{t}_{\textup{\tiny{TV}}}\parenth{#1,#2}}}
\newcommand{\chimix}[2]{\ensuremath{\mathtt{t}_{2}\parenth{#1,#2}}}
\newcommand{\pmix}[3]{\ensuremath{\mathtt{t}_{#1}\parenth{#2,#3}}}
\newcommand{\Ell}{\mathcal{L}}

% big O notation
\newcommand{\Ot}{\widetilde{O}}

% Brackets
\newcommand{\brackets}[1]{\left[ #1 \right]}
\newcommand{\parenth}[1]{\left( #1 \right)}
\newcommand{\bigparenth}[1]{\big( #1 \big)}
\newcommand{\Bigparenth}[1]{\Big( #1 \Big)}
\newcommand{\biggparenth}[1]{\bigg( #1 \bigg)}
\newcommand{\Biggparenth}[1]{\Bigg( #1 \Bigg)}
\newcommand{\braces}[1]{\left\{ #1 \right \}}
\newcommand{\abss}[1]{\left| #1 \right |}
\newcommand{\angles}[1]{\left\langle #1 \right \rangle}
\newcommand{\ceils}[1]{\left\lceil #1 \right \rceil}
\newcommand{\floors}[1]{\left\lfloor #1 \right \rfloor}
\newcommand{\tp}{^\top}

\newcommand{\bmat}[1]{\begin{bmatrix} #1 \end{bmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix} #1 \end{pmatrix}}


% Some vector/matrix norms
\newcommand{\matnorm}[3]{|\!|\!| #1 | \! | \!|_{{#2}, {#3}}}
\newcommand{\matsnorm}[2]{\left|\!\left|\!\left| #1 \right|\!\right|\!\right|_{{#2}}}
\newcommand{\vecnorm}[2]{\left\| #1\right\|_{#2}}


